Learning Minimal Neural Specifications

Formal verification is only as good as the specification of a system, which is also true for neural network verification. Existing specifications follow the paradigm of data as specification, where the local neighborhood around a reference data point is considered correct or robust. While these specifications provide a fair testbed for assessing model robustness, they are too restrictive for verifying any unseen test data points, a challenging task with significant real-world implications. Recent work shows great promise through a new paradigm, neural representation as specification, which uses neural activation patterns (NAPs) for this purpose. However, it computes the most refined NAPs, which include many redundant neurons. In this paper, we study the following problem: Given a neural network, find a minimal (general) NAP specification that is sufficient for formal verification of its robustness properties. Finding the minimal NAP specification not only expands verifiable bounds but also provides insights into which set of neurons contributes to the model's robustness. To address this problem, we propose three approaches: conservative, statistical, and optimistic. Each of these methods offers distinct strengths and trade-offs in terms of minimality and computational speed, making them suitable for scenarios with different priorities. Notably, the optimistic approach can probe potential causal links between neurons and the robustness of large vision neural networks without relying on verification tools, a task existing methods struggle to scale. Our experiments show that minimal NAP specifications use far fewer neurons than those from previous work while expanding verifiable boundaries by several orders of magnitude.

==> Extras.tex <==


\citet{NAPs1} proposes a method to extract and visualize neural activation patterns from pre-trained models.

Those methods share the same idea: prioritizing visualization for explanation. This idea limits what can be evaluated and compared between different methods, since usually a human study is required. Our method tackle the 

They show how different model reacts to different inputs and see how the information on images is processed across the layers. Also, with concepts discovered by analyzing the NAPs of layers, they allow the comparison between models with different architectures for the building-up of classifications across layers. Another similar utilization is, by considering the activation difference between layers as a component to measure if and how the features are evident for or against predictions, providing users with a view of the focus of each layer on images to make decisions with the visualization of activation patterns \citep{zintgraf2017visualizing}. This idea can also apply to domains other than images. Prototypes of Temporally Activated Patterns (PTAP) is a method leveraging activation patterns and their visualization to identify the shapes focused during decision making which helps understand how deep neural networks lean time series data intelligibly \citep{cho2021interpreting}.


In the attempt to explain deep neural network models, few work have focused the attention to the interpretation of the behavior of neural activation patterns \cite{}. 


\textbf{Neural Network Activation Patterns}Neural network activation patterns(NAPs) can help decipher the inner working of neural networks and help individual of interest understand what is learnt by the model. NAPs visualize learned layer concepts. 
    
Current work on NAPs extract similar activation profiles with high-dimensional activation space of a neural network layer and find groups of inputs that are treated similarly. Existing tools can extract NAPs from pre-trained models and provide a visual introspection tool to help analyze NAPs. \cite{NAPs1} 

Neural networks have been playing a significant role in solving various problems. However, the essence of how networks make decisions is still quite unclear to the public, which causes some potential obstacles to adopting neural networks in certain areas such as healthcare and automated drive system. To decipher what has been learned by the inner layer of the neural network, \citet{NAPs1} proposed a methodology and a visual introspection tool to extract neural activation patterns(NAPs) from pre-trained models and analyze them. With the visual analysis of NAPs, we are able to inspect and explain how a model reacts to different inputs and see how the information on images is processed across the layers. Also, with concepts discovered by analyzing the NAPs of layers, they allow the comparison between models with different architectures for the building-up of classifications across layers. Another similar utilization is, by considering the activation difference between layers as a component to measure if and how the features are evident for or against predictions, providing users with a view of the focus of each layer on images to make decisions with the visualization of activation patterns \citep{zintgraf2017visualizing}. This idea can also apply to domains other than images. Prototypes of Temporally Activated Patterns (PTAP) is a method leveraging activation patterns and their visualization to identify the shapes focused during decision making which helps understand how deep neural networks lean time series data intelligibly \citep{cho2021interpreting}.  Apart from analyzing the inner behaviour of a model, activation patterns can also be used for examining the reliability of a decision by checking the similarity of the activation pattern generated during the prediction process with existing patterns extracted from training data, and it can alert to potential misclassification when the similarity is low \citep{cheng2019runtime}.

Verify with NAP. 


==> FigMisclassify1.tex <==
% \begin{figure}[th]
%      \centering
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt6_idx438.pdf}
%          \caption{A testing image from MNIST with ground truth 6, classified as 1}
%          \label{fig:misclsfy_6_to_1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt7_idx129.pdf}
%          \caption{A testing image from MNIST with ground truth 7, classified as 1}
%          \label{fig:misclsfy_7_to_1}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.3\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt9_idx229.pdf}
%          \caption{A testing image from MNIST with ground truth 9, classified as 1}
%          \label{fig:misclsfy_9_to_1}
%      \end{subfigure}
%         \caption{Some interesting test images from MNIST that are misclassified as 1 and also follow the $\NAP$ of class 1.}
%         \label{fig:Misclassify_to_1}
% \end{figure}

==> FigNormdistribution.tex <==
\begin{figure}[t]
     \centering
     % \begin{subfigure}[t]{0.32\textwidth}
     %     \centering        \includegraphics[width=\textwidth]{figures/mnist_L1.png}
     %     \caption{The distribution of $L_1$-norms of all image pairs for each label.}
     %     \label{fig:mnist_L1}
     % \end{subfigure} 
     % \hfill
     \begin{subfigure}[t]{0.48\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/mnist_L2_no_outliers.pdf}
         \caption{The distribution of $L_2$-norms between any two images from the same label. Images of digit (label) 1 are much similar than that of other digits.}
         \label{fig:mnist_L2}
     \end{subfigure}
     \vfill
     \begin{subfigure}[t]{0.48\textwidth}
         \centering         
         \includegraphics[width=0.86\textwidth]{figures/mnist_Linf_no_outliers.pdf}
         \caption{The distribution of $L_\infty$-norms between any two images from the same label. The red line is drawing at 0.05 -- the largest $\epsilon$ used in \citet{vnncomp2021}.}
         \label{fig:mnist_Linf}
     \end{subfigure}
        \caption{Distances between any two images from the same label (class) are quite significant under different metrics of norm.}
        
        \label{fig:mnist_norm}
\end{figure}

==> FigOverlapRatio.tex <==
\begin{figure}[!htb]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap_map_0-0.pdf}
         \caption{$\delta=1.00$}
         \label{fig:overlap ratio 0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap_map_0-01.pdf}
         \caption{$\delta=0.99$}
         \label{fig:overlap ratio 0.01}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.345\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap_map_0-05.pdf}
         \caption{$\delta=0.95$}
         \label{fig:overlap ratio 0.05}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap_map_0-1.pdf}
         \caption{$\delta=0.90$}
         \label{fig:overlap ratio 0.1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap_map_0-15.pdf}
         \caption{$\delta=0.85$}
         \label{fig:overlap ratio 0.1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.345\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/overlap_map_0-5.pdf}
         \caption{$\delta=0.50$}
         \label{fig:overlap ratio 0.5}
     \end{subfigure}
        \caption{Overlap ratio of the dominant pattern of two labels (classes) on a given $\NAP^\delta$. Values in each grid are obtained by $ |N_{col}^{\delta} \bigcap N_{row}^{\delta}|/ |N_{col}^{\delta}|$ where $N_{col}^{\delta}$ is the set of neurons in the dominant pattern for the label (class) of the column of the selected grid with the given $\delta$, $N_{row}$ is the set of neurons in the dominant pattern for the label (class) of the row of the selected grid with the given $\delta$.  }
        \label{fig:overlap ratio}
\end{figure}

==> Fig_visual.tex <==
\begin{figure}[!h]
     \begin{subfigure}[]{0.5\textwidth}
         \centering         \includegraphics[width=0.7\textwidth]{figures/originalNAP.pdf}
         \caption{Linear regions in different colors are determined by weights and biases of the neural network. Points colored either red or green constitute the training set.} 
         \label{fig:linear_regions}
     \end{subfigure}
     \vfill
     \begin{subfigure}[]{0.5\textwidth}
         \centering         \includegraphics[width=0.7\textwidth]{figures/adversial_point.pdf}
         \caption{NAPs are more flexible than $L_\infty$ norm-balls (boxes) in terms of covering verifiable regions.}
         \label{fig:NAP_visual}
         \vfill
     \end{subfigure}
        \caption{Visualization of linear regions and NAPs as specifications compared to $L_\infty$ norm-balls.}
        \label{fig:nap reg}
        % \vspace*{-1cm}
\end{figure}






==> MarabouExample.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=0.8\textwidth]{figures/XNET_vertical.pdf}
         \caption{XNET: A NN that computes the analog XOR function.}
         \label{fig:xornet}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \tiny
         \begin{align*}
             v_0 &= 0.1x_0 - 0.6 x_1 \\
             v_1 &= -4.3x_0 + 4.4 x_1 \\
             v_2 &= 4.2x_0 -4.2x_1 \\
             v_3 &= max(v_0, 0)\\
             v_4 &= max(v_1, 0)\\
             v_5 &= max(v_2, 0)\\
             y_0 &= 0.4v_3 -4.9v_4+3.9v_5+6.7 \\
             y_1 &= -0.4v_3 + 3.9v_4 + 4.6v_5-7.4\\
        % \end{align*}
        % \begin{align*}
             x_0 &\leq 0.1 \wedge x_0 \geq 0.02 \\
             x_1 &\leq 0.1 \wedge x_1 \geq 0.02 \\
             0 &< y_0 - y_1\\
         \end{align*}
         \caption{Marabou's system of constraints for verifying that XNET is 0.04-robust at (0.06, 0.06)}
         \label{fig:marabou_consts}
     \end{subfigure}
     \hfill
     %-------------------------------------
    \begin{subfigure}[b]{0.35\textwidth}
         \centering
         \tiny
         \begin{align*}
             v_0 &= 0.1x_0 - 0.6 x_1 \\
             v_1 &= -4.3x_0 + 4.4 x_1 \\
             v_2 &= 4.2x_0 -4.2x_1 \\
             v_3 &= v_0 \\
             v_4 &= max(v_1, 0) \\
             v_5 &= 0 \\
             y_0 &= 0.4v_4 -4.9v_5+3.9v_6+6.7 \\
             y_1 &= -0.4v_4 + 3.9v_5 + 4.6v_6-7.4 \\
            x_0 &\leq 0.3 \wedge x_0 \geq 0 \\
             x_1 &\leq 0.3 \wedge x_1 \geq 0 \\
             v_0 &\geq 0 \\
             v_2 &\leq 0
         \end{align*}
         \caption{Check if $\cP_{\ell=1}=((z_0),())$ and $\cP_{\ell=0} = ((),(z_2))$ are non-ambiguous in the first quadrant using Marabou}
         \label{fig:marabou_wiht_relu_consts}
     \end{subfigure}
     \hfill
        \caption{Using Marabou to verify NAP properties of XNET.}
        \label{fig: XOR_example}
\end{figure}

==> NAP_overlapping.tex <==
\begin{table}[th!]
\caption{The maximum overlap ratio for each label (class) on a given $\NAP^\delta$ for MNIST. Each cell is obtained by $\max_i |N_{col}^{\delta} \bigcap N_i^{\delta}|/ |N_{col}^{\delta}|$ where $N_{col}^{\delta}$ is the set of neurons in the dominant pattern for the label (class) in the header of the column of the selected cell with the given $\delta$, $N_i$ is the set of neurons in the dominant pattern for the label (class) $i$ with the given $\delta$.} 
\label{tab:mnist_max_overlap_ratio}
\begin{center}
\begin{tabular}{ |l || r r r r r r r r r r| }
\hline
& 0& 1& 2& 3& 4& 5& 6& 7& 8& 9\\
\hline\hline
1.00&0.959 &0.928 &0.963 &0.966 &0.972 &0.973 &0.930 &0.965 &0.957 &0.981\\ 
 \hline
0.99&0.844 &0.834 &0.911 &0.901 &0.881 &0.898 &0.895 &0.884 &0.880 &0.908\\ 
 \hline
0.95&0.864 &0.885 &0.909 &0.904 &0.915 &0.908 &0.899 &0.897 &0.890 &0.893\\ 
 \hline
0.90&0.877 &0.900 &0.910 &0.901 &0.921 &0.910 &0.890 &0.899 &0.900 &0.901\\ 
 \hline
0.85&0.876 &0.904 &0.904 &0.900 &0.919 &0.913 &0.893 &0.907 &0.904 &0.900\\ 
 \hline
0.75&0.893 &0.922 &0.913 &0.912 &0.928 &0.925 &0.905 &0.916 &0.916 &0.913\\ 
 \hline
0.50&0.903 &0.905 &0.925 &0.923 &0.926 &0.923 &0.907 &0.918 &0.927 &0.927\\ 
 \hline
\end{tabular}
\end{center}
\end{table}

==> Problem.tex <==
\section{Problem FORMULATION and Naive Approaches}
\label{problemformulation}

==> abstract.tex <==

Despite Deep Neural Network's state-of-the-art performance, they make mistakes and suffer from adversarial attacks. Thus, being able to trust the classification for a given input is an important research area. While numerous methods have been developed to provide explanations for individual classifications with a range of different justifications, they can only establish a \emph{correlation} between a prediction and an explanation. In this work, we address a fundamental question: can we prove the \emph{causality} of an explanation: if a single input $x$ is classified by a neural net $N$ as $y$ because of a predicate reason $P(x)$ (written $P(x) \implies N(x) = y$), does that mean all inputs that satisfies $P$ will have the same classification $y$? To this end, we introduce a novel encoding for popular explanation methods and extend Marabou, a state-of-the-art NN verifier, to verify their causality. 
When the explanation cannot be used to explain the predictions in all of the input space, we quantify how many test examples can be explained by each method, thus providing valuable metrics to guide the choice between different explanations. Furthermore, we show that explanations can also be used to strengthen neural networks' robustness, even if they do not cover the whole input space. Finally, we empirically validate our technique using various real-world datasets, model classes, and explanation functions. By providing the first study on verifying neural networks' explanation, our work provides a framework to evaluate existing explanation methods, and guides the way for researching new ones.

==> case_study.tex <==

\section{Case Study: the Iris dataset classification}
\label{sec:case_study}
% \input{Fig_visual.tex}




\subsection{Calculating the change in volume from the original NAP to the minimal NAP specification.}





\subsection{Understanding Double Descent via the Lens of Minimal NAP Specification}


==> gradient_search.tex <==

\subsection{Gradient-guided Search}

We introduce another approach called \textsc{Gradient\_Search} to identify mandatory neurons. Similar to \textsc{Adversarial\_Prune}, \textsc{Gradient\_Search} avoids costly interactions with the verification tool. Instead, it leverages gradient estimations to analyze the structure of $\mathbf{F}$. 




Recall our definition of a neural network in Section \ref{sec:NN_basic}, where the output $\mathbf{F}(x)$ can be seen as a function of the post-activation value of any internal neuron $\hat{z}_i^{(l)}$. We denote this function as $\mathbf{F}(\hat{z}(x))$, omitting $i$ and $l$ for simplicity. The function $\mathbf{F}(\hat{z})$ is non-linear and operates within an input range of $\hat{z} \in [0, +\infty)$. It is worth noting that the gradient $\frac{\partial \mathbf{F}}{\partial \hat{z}}$ can provide valuable insights into the local structure of $\mathbf{F}$. This insight may help determine the necessity condition of mandatory neurons by checking if there exists a $\hat{z}$ such that $\mathbf{F}(\hat{z}) < 0$ for the corresponding neuron. To be more specific, given some sampled data $\hat{z}_1, \ldots, \hat{z}_n$, we can compute their corresponding function values $\mathbf{F}(\hat{z}_1), \ldots, \mathbf{F}(\hat{z}_n)$ along with their gradients $\frac{\partial \mathbf{F}}{\partial \hat{z}}|_{\hat{z}_1}, \ldots, \frac{\partial \mathbf{F}}{\partial \hat{z}}|_{\hat{z}_n}$. Then if there exists a $\hat{z}_j$ such that $|\mathbf{F}(\hat{z}_j)|$ is sufficiently small, yet the norm of its gradient $|\frac{\partial \mathbf{F}}{\partial \hat{z}}|_{\hat{z}_j}|$ is significantly large, then it is very likely that $\mathbf{F}$ will go below zero nearby, as illustrated in Figure \ref{fig:gradient_f}. Then, if we happen to know that the corresponding neuron $N_{i,l}$ is in state $\mathbf{0}$, it is highly likely that $N_{i,l}$ is mandatory. Conversely, if a neuron $N_{i,l}$ is in state $\mathbf{1}$, and we sample an $x$ such that $\hat{z}_i^{(l)} = 0$ and $\mathbf{F}(x) < 0$, we immediately recognize that the neuron is mandatory. Algorithm \ref{alg:Heuristics} presents pseudocode for estimating whether a neuron is mandatory based on the discussions above.




% As we illustrate, both \textsc{Gradient\_Search} and \textsc{Adversarial\_Prune} provide estimates of minimal NAPs without call $\mathcal{V}$. However, these approaches can also work in $\mathcal{V}$ dependent fashion. By validating estimates
%  using the verification tool $\mathcal{V}$. If verification fails, \textsc{Adversarial\_Prune} can use a new set of adversarial examples and take the union of the new mandatory neurons with the current set. Similarly, \textsc{Gradient\_Search} can adjust the hyperparameters $\beta$ and $\gamma$ and take the union of the new results with the current set. Through these iterative interactions with $\mathcal{V}$, both methods are expected to converge on an estimate of minimal NAP specifications with significantly fewer calls to $\mathcal{V}$.



As we demonstrate, both \textsc{Gradient\_Search} and \textsc{Adversarial\_Prune} can estimate minimal NAPs without calling the verification tool $\mathcal{V}$. However, these methods can also operate in a $\mathcal{V}$-dependent manner. By validating the estimates using  $\mathcal{V}$, if verification fails, \textsc{Adversarial\_Prune} can generate new adversarial examples and combine the newly identified mandatory neurons with the current set. Likewise, \textsc{Gradient\_Search} can sample new data and merge the updated mandatory neurons into the existing set.
Through these iterative interactions with $\mathcal{V}$, both methods are expected to converge on minimal NAP specifications with significantly fewer calls to $\mathcal{V}$.




% adjust the hyperparameters $\beta$ and $\gamma$





% Both \textsc{Gradient\_Search} and \textsc{Adversarial\_Prune} provide estimates of minimal NAPs. These estimates can be validated using the verification tool $\mathcal{V}$. If verification fails, \textsc{Adversarial\_Prune} can employ a new set of adversarial examples and combine the resulting mandatory neurons with the current set. Similarly, \textsc{Gradient\_Search} can adjust the hyperparameters $\beta$ and $\gamma$ to refine its estimates. Through these iterative interactions with $\mathcal{V}$, both methods are expected to converge on an estimate of minimal NAP specifications with significantly fewer calls to $\mathcal{V}$.










% Both \textsc{Gradient\_Search} and \textsc{Adversarial\_Prune} provide us  estimates of mnimial NAPs. In addition, their estmats can be checked by calling the verfication tool $\mathcal{V}$. If fails, \textsc{Adversarial\_Prune} could use an other set of adversial examples, and take union of new manduatoy neruins with current ones, \textsc{Gradient\_Search} could work in the simailetr fashion by altering hyperpaprametes $\beta$ and $\gamma$, in this intertaive interactionts with $\mathcal{V}$, they are expected to find an esrtimate of minimal NAP specfications with much less calls to $\mathcal{V}$.


% In this way, they can be used to learn minimal NAP specfications



% be used 
% as initial guess

% together. Taking the intersection of their estimated results may provide us with a better overall estimate. In addition, the estimated mandatory neurons can serve as an initial starting point in our statistical versions of the \textsc{Refine} and \textsc{Coarsen} approaches introduced in Section \ref{sec:stat_approach}.

% Our experimental results regarding these two estimation approaches indicate a notable trend: neurons from deeper layers are more likely to be mandatory. This observation aligns with commonly-held beliefs that deeper neurons are generally linked to high-level feature representation, and thus play a more important role than shallow neurons in final classification decisions. 



\begin{algorithm2e}[H]
    \caption{\textsc{Gradient\_Search}}
    \label{alg:Heuristics}
    \small
    \DontPrintSemicolon
    \SetKwProg{Fn}{Function}{}{end}
    \SetKwFunction{Coarsen}{Coarsen}
    \KwIn{The neural network $N$, the input dataset $X$, and thresholds $\beta$, $\gamma$ }
    \KwOut{A collection of mandatory neurons}
     
    \Fn{Gradient\_Search($N$, $X$, $\beta$, $\gamma$)}{
        $Mand \leftarrow \emptyset$ ; $P \leftarrow \widetilde{\mathcal{A}}(N) $ \;
        \For{$N_{i, l}$ \textbf{in} $N$}{ 
            \For{$x_{j}$ \textbf{in} $X$}{ 
             $\hat{z}_j \leftarrow \hat{z}_i^{(l)}(x_j)$ \;             
             \uIf{$\hat{z}_j > 0$ }{
                  \uIf{ $|\mathbf{F}(\hat{z}_j)| < \beta$ and $|\frac{\partial \mathbf{F}}{\partial \hat{z}_i^{(l)}}|_{\hat{z}_j}| > \gamma$ and $P_{i, l} == \mathbf{0}$}{$Mand \leftarrow Mand \cup \{N_{i, l}\}$   \tcc*{Neuron is in state $\mathbf{0}$, can't coarsen} } }
            
        \Else{
            \uIf{$\mathbf{F}(\hat{z}_j) < 0$ and $P_{i, l} == \mathbf{1}$}{
            $Mand \leftarrow Mand \cup \{N_{i, l}\} $
            \tcc*{Neuron is in state $\mathbf{1}$, can't coarsen} } 
            }
        }
        }  
        \Return $Mand$\;
        }    
\end{algorithm2e}



% Assuming we have access to $\mathbf{F}(\hat{z})$ and $\frac{\partial \mathbf{F}}{\partial \hat{z}}$ on some samples $\hat{z}_1,...,\hat{z}_n$, if all values of $\mathbf{F}(\hat{z})$ are greater than 0 and the gradients $\frac{\partial \mathbf{F}}{\partial \hat{z}}|_{\hat{z}_i}$ are close to 0, then it is very likely that $\mathbf{F}(\hat{z}) \geq 0$ for the input range $(0,+\infty)$.  On the other hand, if the gradients on certain sample data are large, i.e., $\mid \frac{\partial \mathbf{F}}{\partial \hat{z}}|_{\hat{z}_j} \mid \gg 0$, it is likely that $\mathbf{F}(\hat{z})$ could go lower than 0 somewhere in  $(0,+\infty)$. When this happens to a neuron in state $\mathbf{0}$, it suggests the neuron is likely to be a mandatory neuron, as described in Algorithm \ref{alg:Heuristics}. 








% This observation leads us to a valuable heuristic: prioritizing deeper neurons over shallower ones as we iterate through neurons in our implementations of the \textsc{Refine} and \textsc{Coarsen} algorithms.

% The \textsc{Gradient\_Heuristics} algorithm allows us to efficiently infer mandatory neurons based on their necessary conditions and will serve as an important heuristic in our statistical learning approaches.



% \For {$x_{j}$ \textbf{in} $X$ {}


            % \For {$x_{j}$ \textbf{in} $X$ {}

% $\mathbf{G}>0$

% $\frac{\partial \mathbf{G}}{\partial \hat{z}_i^{(l)}}$ is close to 0 and $\mathbf{G}>0$, then 



% with respect to $\hat{z}_i^{(l)}$ $\frac{\partial \mathbf{G}}{\partial \hat{z}_i^{(l)}}$

% \frac{\partial \mathbf{G}}{\partial \hat{z}_i^{(l)}}




% We know 
% This 


% For the neurons that 

% \begin{align}
% \label{eq:stat_func}
%  \widetilde{\mathcal{A}}(N_{i, l}, X) =
% \begin{cases}
%   \mathbf{0} & \text{if } \frac{|\{x_j|\ddot{\mathcal{A}}(N_{i, l}, x_j ) = \mathbf{0}, \text{ } x_j \in X\}|}{|X|} \geq \delta \\
%   \mathbf{1} & \text{if } \frac{|\{x_j|\ddot{\mathcal{A}}(N_{i, l}, x_j ) = \mathbf{1}, \text{ } x_j \in X\}|}{|X|} \geq \delta \\ 
%   \mathbf{*} & \text{otherwise}\\ 
% \end{cases}
% \end{align}


% refined to $\mathbf{1}$ or $\mathbf{0}$.



% Fortunately, we can leverage the computation of gradient flows in neural networks to estimate $M$. 
% Recall the robustness verification given a NAP specification $P^c$ is equivalent to showing that $\mathbf{F}_c(x) - \mathbf{F}_k(x) > 0$ for input $x$ falls into $P^c$ specified region. We know that 


% Suppose a neuron $N_{i,l}$ in $P^c$ is abstracted into $\mathbf{1}$, i.e., $\hat{z}_i^{(l)} \in (0,+\inf)$, if $N_{i,l} \in M$, then 







% Formally, we have:
% \begin{align}
%     \forall x \in R_{P^{c}} \quad \forall k \in C \text{ s.t. } k\neq c  \quad  \mathbf{F}_c(x) - \mathbf{F}_k(x) > 0
% \end{align}
% in which 
% \begin{align}
%     R_{P^{c}}= \{ x \mid {\mathcal{A}(N,x) \preccurlyeq P^c}  \}  
% \end{align}

% The most refined NAP $\widetilde{\mathcal{P}}$ clearly


% -
% We take the gradient of $\mathbf{F}_c(x) - \mathbf{F}_k(x)$ with respect to the post-activation value of an arbitrary neuron $\hat{z}_i^{(l)}(x)$. 

% \begin{align}
% \frac{\partial \mathbf{G}}{\partial \hat{z}_i^{(l)}}
% \end{align}



% can then be reduced to 

% Intuitively, the \textsc{refine} and \textsc{coarsen} algorithms 











       
% Since adversarial attacks have been extensively studied, offering a wealth of methods that we can leverage. We could easily idenr



% leverages the existence of adversarial examples to efficiently prune the search space of NAPs, avoiding costly interactions with the verification tool.


% When an adversarial example $x'$ is found, it immediately indicates the NAP $\ddot{\mathcal{A}}(N, x' )$ fails verification, i.e., $\mathcal{V}(\ddot{\mathcal{A}}(N, x' )) = 0$. Consequently, it also suggests any NAPs that subsume $\ddot{\mathcal{A}}(N, x' )$ fail verification as well. For instance, suppose an adversarial example $x'$ is found for a simple four-neuron neural network and $\ddot{\mathcal{A}}(N, x' )$ is $\{\mathbf{1},\mathbf{0},\mathbf{1},\mathbf{0}\}$, we can effectively rule out $\{\mathbf{1},\mathbf{0},\mathbf{1},\mathbf{*}\}$, $\{\mathbf{1},\mathbf{0},\mathbf{*},\mathbf{*}\}$, $\{\mathbf{1},\mathbf{*},\mathbf{*},\mathbf{*}\}$, and $\{\mathbf{*},\mathbf{*},\mathbf{*},\mathbf{*}\}$. In the context of finding the minimal NAP specification, adversarial examples can be used to identify mandatory neurons. Formally, in a NAP, for a neuron $N_{i, l}$, we check: 

% \begin{enumerate}
%     \item If $N_{i, l}$ is in state $\mathbf{0}$,  if an adversarial example $x'$ is found, and produce the NAP  $\ddot{\mathcal{A}}(N_{i, l}, x ) = 0$,
    
%     trigger a NAP,
    
%     it implies when $ \hat{z}_i^{(l)}(x) = 0, \mathbf{F}(x) \geq 0$. In addition, $\exists x \text{ s.t. } \hat{z}_i^{(l)}(x) > 0, \mathbf{F}(x) < 0$.
%     \item If $N_{i, l}$ is in state $\mathbf{1}$, it implies $\forall x \text{ s.t. } \hat{z}_i^{(l)}(x) > 0, \mathbf{F}(x) \geq 0$.  In addition, when  $ \hat{z}_i^{(l)}(x) = 0, \mathbf{F}(x) < 0 $. 
% \end{enumerate}









% \section{Statistical Learning Approaches}
% \label{sec:stat_approach}
% In this section, we introduce two new algorithms that address the minimal NAP specification problem. While they share the same overarching concept as \textsc{refine} and \textsc{coarsen}, these methods employ sampling and statistical learning principles to efficiently learn a minimal NAP specification. Recall that the set of mandatory neurons $M$ is the union of all neurons that appears in any minimal specification and is an upper bound of the largest minimal specification.
% While they share the same overarching concept as \textsc{refine} and \textsc{coarsen}, these methods employ various heuristics and statistical learning principles to efficiently find a minimal NAP specification. 
% While the \textsc{refine} and \textsc{coarsen} algorithms can find 
% minimal NAP specifications, they are not efficient. In this section, we introduce two statistical learning approaches
% : \textsc{Statrefine} and \textsc{Statcoreasn}, for finding minimal NAP specifications. While 
% Both approaches share the same idea as the \textsc{refine} and \textsc{coarsen} algorithms presented in the previous section. More specifically, \textsc{Statrefine} starts from the coarsest NAP and then refines it, while \textsc{Statcoreasn} operates in the opposite direction. However, we show that \textsc{refine} and \textsc{coarsen} algorithms    
% abstractions. The two algorithms are STATREFINE, which refines an abstraction by iteratively adding components (Section 4.1) and ACTIVECOARSEN, which coarsens an abstraction by removing components.
% At a high level, these two algorithms parallel their deterministic counterparts presented in the previous section. However, there are two important distinctions worth noting: (i) the machine learning algorithms find a minimal abstraction much more effectively by exploiting sparsity, the property that a minimal abstraction contains a small fraction of the full set of components; and (ii) randomization is used to exploit this sparsity.
% As we discussed before, minimal NAP specifications are formed by certain sets of neurons that abstract to binary states, i.e., $\mathbf{1}$ or $\mathbf{0}$. Therefore
% \subsection{The Statistical Refine Approach} 
% Mandatory neurons are crucial for forming NAP specifications, as their binary states play a critical role in determining the neural network's robustness performance. We leverages this property to find mandatory neurons statistically. To be more specific, suppose we sample some NAPs $P_1, P_2, \ldots, P_n$ from the NAP family $\mathcal{P}$. For those NAPs that qualify as specifications (i.e., $\mathcal{V}(P) = 1$), mandatory neurons should appear more frequently in them than in those NAPs that fail the verification tool (i.e., $\mathcal{V}(P) = 0$). 

% Based on this insight, we propose an approach called \textsc{Sample\_Refine} that relies on non-repetitive sampling to identify mandatory neurons for solving the minimal NAP problem. We start with the coarsest NAP and iteratively collect the most probable mandatory neurons. In every iteration, we sample $k$ NAPs by refining unvisited neurons with some probability $\theta$. The sampled NAPs are then fed to the verification tool, and the neuron that appears most frequently in verifiable NAPs is the most probable mandatory neuron in this iteration. The neuron is marked as visited, and the process stops when either we collect $s$ neurons (assuming that $s$ is known), or the current mandatory neurons form a NAP specification $P$, i.e., $\mathcal{V}(P) = 1$. Finally, we return the learned NAP, obtained by applying $\widetilde{\mathcal{A}}$ to the collected neurons. The algorithm~\ref{alg:samplerefine} provides an overview of the above procedure.


% It is worth noting that \textsc{Sample\_Refine} doesn't guarantee correctness, as we may end up collecting only the $s$ most probable mandatory neurons, which may not be sufficient to form a specification. Another concern regarding this algorithm is sampling efficiency, specifically the potential for the number of samples required to grow exponentially with the size of the minimal NAP specification $s$. To understand why this is problematic, consider a scenario where the only minimal NAP specification $P$ consists of all mandatory neurons; in this case, all $|M|$ neurons must be selected for $P$ to be learned. If $\theta$ is set to a constant value, then the expected number of samples needed to obtain the NAP specification is $(\frac{1}{\theta})^{|M|}$. To address this, we set $\theta = \left(\frac{|M|}{|M|+1}\right)^{|M|}$. This choice ensures that the sampling efficiency is polynomial in both $|M|$ and $s$, as proven in Theorem \ref{thm:theorem_refine}. Please refer to the proof in the Appendix \ref{appendix:proof_stats}.  In addition, Theorem \ref{thm:theorem_refine} also shows that with high probability, a mandatory neuron will be found with $O(log|N|)$ calls to $\mathcal{V}$. 


% \begin{algorithm2e}[H]
%     \caption{\textsc{Sample\_Refine}}
%     \label{alg:samplerefine}
%     \small
%     \DontPrintSemicolon
%     \SetKwProg{Fn}{Function}{}{end}
%     \SetKwFunction{Coarsen}{Coarsen}
%     \KwIn{The neural network $N$, the probability $\theta$, sample size $k$, and the size $s$}
%     \KwOut{A minimal NAP specification $P$}
    
%     \Fn{Sample\_NAPs($unvisited$, $\theta$)}{
%         $P \leftarrow \dot{\mathcal{A}}(N)$ \tcc*{Use the coarsest NAP as a blank template}
%         \For{$N_{i, l}$ \textbf{in} $unvisited$}{
%             $rand \leftarrow \text{random}(0,1)$ \;
%             \uIf{$rand \leq \theta$}{
%                 $P \leftarrow \widetilde{\Delta}(N_{i, l})$ \tcc*{Refine unvisited neurons using $\widetilde{\Delta}$ with probability $\theta$}
%             }
%         }
%         \Return $P$\;
%     }

%     \Fn{Sample\_Refine($visited$, $\theta$, $k$, $s$)}{
    
%     \While{$|visited| < s \text{ and }  \mathcal{V}(P) == 0 $ }{
%         $unvisited \leftarrow N \setminus visited$ \;
%         $ctr = dict()$ \tcc*{Create a counter for each neuron in $unvisited$} 
%         \For{$\_$ \textbf{in} $range(k)$}  {
%             $P \leftarrow Sample\_NAPs(unvisited, \theta)$ \tcc*{Sample $k$ NAPs} 
%             \For{$N_{i, l}$ \textbf{in} $unvisited$}{
%                 \uIf{$P_{i,l} == \widetilde{\mathcal{A}}(N_{i, l})$ \textbf{and} $\mathcal{V}(P) == 1$}{
%                     $ctr[N_{i, l}]$ += 1 \tcc*{Count successful NAPs for each neuron}
%                 }
%             }
%         }
%         $N_{mad} \leftarrow \argmax_{N_{i,l} \in unvisited} \{ctr[N_{i, l}]\}$ \tcc*{Pick potential mandatory neuron} 
%         $visited \leftarrow visited \cup \{N_{mad}\}$ \;
%     }
%     \Return $\widetilde{\mathcal{A}}(visited)$\;
%     }
    
%     $P \leftarrow \widetilde{\mathcal{A}}(N)$\;
%     \uIf{$\mathcal{V}(P) == 0$}{
%         \Return $None$ \tcc*{Return None if the most refined NAP fails verification}
%     }
%     \Else{
%         \uIf{heuristics}{
%             $visited \leftarrow Gradient\_Search(N) \cap Adversarial\_Prune(N) $ 
%         }
%         \Else{
%             $visited \leftarrow \emptyset$ \tcc*{Start from the coarsest NAP}
%         }
%         $Sample\_Refine(visited, \theta, k, s)$\;
%     }
    
% \end{algorithm2e}



% % Theorem \ref{thm:theorem_refine} shows that with high probability, a mandatory neuron will be found with $O(log|N|)$ calls to $\mathcal{V}$. 

% % It's important to note that \textsc{Sample_Refine} does not guarantee correctness, as it only selects the $s$ most probable mandatory neurons. Theorem \ref{thm:theorem_refine} demonstrates that with high probability, a mandatory neuron can be found with $O(\log|N|)$ calls to $\mathcal{V}$. Another concern regarding this algorithm is its sampling efficiency, which can lead to an exponential increase in the number of samples required relative to the size of the minimal NAP specification $s$. To illustrate this issue, consider a scenario where the minimal NAP specification $P$ contains all mandatory neurons. In such a case, all $|M|$ neurons must be included in $P$ for it to be learned. If $\theta$ is set to a constant value, the expected number of samples needed to find one that can be verified is $(\frac{1}{\theta})^{s}$.





% % We also aim to demonstrate that the number of calls is polynomial in terms of $|M|$ and $s$. Fortunately, this can be achieved by carefully setting the sampling probability $\theta$. To give a intuition,
% % suppose we find a minimal NAP $P$ with size $s = |M|$ is a specification, i.e., \( \mathcal{V}(P) = 1 \) if and only if $P=\widetilde{\mathcal{A}}(P)$. In \textsc{Sample\_Refine}, since each neuron is selected independently with probability $\theta$. If $\theta$ is constant throughout the iterations, the expected number of samples needed to reach one that can be verified is $(\frac{1}{\theta})^{s}$. We show that a proper refinement probability \( \theta \) allows $k$ to be polynomial with respect to $|M|$ while constraining the number of calls to $\mathcal{V}$. 

% \begin{theorem}
% \label{thm:theorem_refine}
% With probability $\theta = |(\frac{|M|}{|M|+1})|^{|M|} $, \textsc{Sample\_Refine} has \( 1 - \delta \) probability of outputting a minimal NAP specification with $\Theta\left(|M|^2(\log|N| + \log(s/\delta))\right)$ examples each iteration and \( O(s|M|^2(\log|N| + \log(s/\delta))) \) total calls to \( \mathcal{V} \).
% \end{theorem}


% We will include the proof in the appendix. 

% \begin{proof}
% Let $P$ be the NAP returned by \textsc{coarsen}. We aim to show that any $P'$ smaller than $P$ results in $\mathcal{V}(P') = 0$. To construct such a smaller $P'$, we would need to refine some $N_{i, l}$ using $\widetilde{\mathcal{A}}$, i.e., $P' := \widetilde{\mathcal{A}}(N_{i, l}) \cup P \setminus P_{i,l}$. According to the algorithm, $\mathcal{V}(P') = 0$.  In the worst case, the algorithm needs to iterate through each neuron in $N$, resulting in a runtime complexity of $\mathcal{O}(|N|)$.
% \end{proof}





% \subsection{The Statistical Coarsen Approach}
% The \textsc{Coarsen} algorithm begins with the most refined NAP and progressively coarsens each neuron until the verification process fails. Enhancing the algorithm's performance is possible by coarsening multiple neurons during each iteration. However, a fundamental question emerges: How do we determine which set of neurons to coarsen in each round? 

% We present \textsc{Sample\_Coarsen} to answer this question. In this approach, we assume that each neuron is independent of the others and select neurons to coarsen in a statistical manner. Specifically, in each iteration, we randomly coarsen a subset of refined neurons in the current NAP simultaneously to see if the new NAP can pass verification. We repeat this process until the NAP size reaches $s$. Algorithm \ref{alg:samplecoarsen} provides the pseudocode for \textsc{Sample\_Coarsen}.


% \vspace{20pt}





% count the number of NAPs that passed verification. For the neuron that enable;e


% neurons




% In every iteration, the most probable mandatory neuron is the 

% The sampling is non-repetitive and 

% and probability $\theta$, and 



% \textsc{StatRefine} identifies dependent components by sampling \( n \) independent random abstractions and running the static analysis $\mathcal{V}$ on them. The component $j$ associated with the most number of proven queries is then added to the abstraction, and we iterate. The pseudocode of the algorithm is given in Figure \ref{alg:statrefine}. STATREFINE relies on correlations with the output of $\mathcal{V}$ to find dependent components. As Theorem 2 will show, with high probability, a dependent component can be found with $n$ calls to $\mathcal{V}$, where $n$ is only logarithmic in the total number of components $|\mathbb{J}|$.



% We call a component $j \in \mathbb{J}$ dependent if $j$ appears in any minimal abstraction. Let \( D \subset \mathcal{J} \) be the set of dependent components and let \( d = |D| \). Note that \( D \) is the union of all minimal abstractions. Define \( s \) to be the size of the largest minimal abstraction, observing that \( s \leq d \). 





% \rebecca{derive our own gradient for alpha?}

% Let \( d \) be the number of dependent components in \( \mathbb{J} \) and \( s \) be the size of the largest minimal abstraction. Suppose we set the refinement probability \( \alpha = \left(\frac{d}{d+1}\right)^d \) and obtain \( n = \Theta\left(d^2(\log|\mathbb{J}| + \log(s/\delta))\right) \) training examples from \( F \) each iteration. Then with probability \( 1 - \delta \), \textsc{StatRefine}(\(\emptyset\)) outputs a minimal abstraction with \( O(sd^2(\log|\mathbb{J}| + \log(s/\delta))) \) total calls to \( \mathcal{V} \).






% \begin{algorithm}
% \caption{Refinement via Statistical Learning}
% \label{alg:statrefine}
% \begin{algorithmic}
% \STATE \textbf{Parameters:}
% \STATE \hspace{\algorithmicindent} $\alpha$: refinement probability
% \STATE \hspace{\algorithmicindent} $s$: size of largest minimal abstraction
% \STATE \hspace{\algorithmicindent} $n$: number of training examples per iteration
% \\
% \STATE \textbf{function} SAMPLE$(\alpha, a^L, a^U)$:
% \STATE \hspace{\algorithmicindent} $a \gets a^L$
% \STATE \hspace{\algorithmicindent} \textbf{for} each component $j \in a^U \setminus a^L$:
% \STATE \hspace{\algorithmicindent} \hspace{\algorithmicindent} $a_j \gets 1$ with probability $\alpha$
% \STATE \hspace{\algorithmicindent} \textbf{return} $a$
% \STATE \textbf{end function}
% \\
% \STATE \textbf{function} STATREFINE$(a^L)$:
% \STATE \hspace{\algorithmicindent} \textbf{if} $F(a^L) = 0$ \textbf{or} $|a^L| = s$: \textbf{return} $a^L$
% \STATE \hspace{\algorithmicindent} \textbf{for} $i = 1$ \textbf{to} $n$: \COMMENT{create training examples}
% \STATE \hspace{\algorithmicindent} \hspace{\algorithmicindent} $a^{(i)} \gets$ SAMPLE$(\alpha, a^L, \mathbb{J})$
% \STATE \hspace{\algorithmicindent} \hspace{\algorithmicindent} \textbf{for} each $j \not\in a^L$: \COMMENT{compute a score for each component}
% \STATE \hspace{\algorithmicindent} \hspace{\algorithmicindent} \hspace{\algorithmicindent} $n_j \gets |\{ i : a^{(i)}_j = 1, F(a^{(i)}) = 0\}|$
% \STATE \hspace{\algorithmicindent} \hspace{\algorithmicindent} $j^* \gets \arg\max_{j \not\in a^L} n_j$ \COMMENT{choose best component}
% \STATE \hspace{\algorithmicindent} \textbf{return} STATREFINE$(a^L \cup \{j^*\})$
% \STATE \textbf{end function}
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
% \caption{Coarsening via Active Learning}
% \label{alg:activecoarsen}
% \begin{algorithmic}
% \STATE \textbf{ACTIVECOARSEN}(\(a^U\)):

% \STATE \textbf{Parameters:}

% \STATE \hspace{\algorithmicindent} $\alpha$: refinement probability

% \STATE \hspace{\algorithmicindent} $s$: size of largest minimal abstraction
% \\
%     \IF{\(|a^U| \leq s + 1\)}
%         \RETURN \textsc{ScanCoarsen}(\(\emptyset, a^U\))
%     \ENDIF
%     \STATE \(a \gets \textsc{Sample}(\alpha, \emptyset, a^U)\)
%     \IF{\(\mathcal{V}(a) = 0\)}
%         \STATE \COMMENT{run static analysis}\\
%         \RETURN \textsc{ActiveCoarsen}(\(a\)) \COMMENT{reduced}
%     \ELSE
%         \RETURN \textsc{ActiveCoarsen}(\(a^U\)) \COMMENT{try again}
%     \ENDIF
% \end{algorithmic}
% \end{algorithm}


% \subsection{The Statistical Coarsen Approach}
% The \textsc{Coarsen} algorithm begins with the most refined NAP and progressively coarsens each neuron until the verification process fails. Enhancing the algorithm's performance is possible by coarsening multiple neurons during each iteration. However, a fundamental question emerges: How do we determine which set of neurons to coarsen in each round? 

% We present \textsc{Sample\_Coarsen} to address this question. In this approach, we assume that each neuron is independent of the others and select neurons to coarsen in a statistical manner. Specifically, in each iteration, we randomly coarsen a subset of refined neurons in the current NAP simultaneously to see if the new NAP can pass verification. We repeat this process until the NAP size equals $s$. Algorithm \ref{alg:samplecoarsen} provides the pseudocode for \textsc{Sample\_Coarsen}.




% Theorem 3 (Properties of ACTIVECOARSEN). Let s be the
% size of the largest minimal abstraction. If we set the refinement probability α = e
% −1/s, the expected number of
% calls to the analysis F made by ACTIVECOARSEN(J) is
% O(s log |J|).




% \textbf{Theorem 3 (Properties of \textsc{ActiveCoarsen})}. Let \(s\) be the size of the largest minimal abstraction. If we set the refinement probability \(\alpha = e^{-1/s}\), the expected number of calls to the analysis \(\mathcal{V}\) made by \textsc{ActiveCoarsen}(\(\mathbb{J}\)) is \(O(s \log |\mathbb{N}|)\).


% We now present our second machine learning algorithm, \textsc{ActiveCoarsen}. Like \textsc{ScanCoarsen}, it starts from the finest abstraction \(\mathbb{J}\) and tries to remove components from \(\mathbb{J}\). But instead of doing this one at a time, \textsc{ActiveCoarsen} tries to remove a random constant fraction of the components at once. As we shall see, this allows us to hone in on a minimal abstraction much more quickly.

% The pseudocode of the algorithm is given in Figure 3. It maintains an upper bound \(a^U\) which is guaranteed to prove the query. It repeatedly tries random abstraction \(a \leq a^U\) until \(a\) can prove the query (\(F(a) = 0\)). Then we set \(a^U\) to \(a\) and repeat.

% Recall that \textsc{ScanCoarsen}, which removes one component at a time, requires an exorbitant \(O(|\mathbb{J}|)\) calls to the static analysis. The key idea behind \textsc{ActiveCoarsen} is to remove a constant fraction of components each iteration. Then we would hope to need only \(O(\log_{1/\alpha} |\mathbb{J}|)\) iterations.





% Similar to \textsc{Sample\_Refine}, \textsc{Sample\_Coarsen} also faces the same challenge related to sample efficiency. To better illustrate this, suppose a minimal NAP specification $P$ with size $s$ can be found after one iteration of refinement. Then, the probability of selecting the exact number of $s$ mandatory neurons in $P$ is $\theta^{s}$. Consequently, if $\theta$ is set to a constant value, the expected number of samples needed to find the NAP is $(\frac{1}{\theta})^{s}$.  Unlike \textsc{Sample\_Refine}, we know the refinement will always ensure the resulting NAP can pass verification. So, once such a NAP is learned, we can narrow down the estimated mandatory neurons by an expected factor of $\theta$. In this way, the expected number of samples and the expected number of iterations are inversely related, yet their product is the total number of calls to $\mathcal{V}$. We demonstrate that by setting $\theta = e^{-\frac{1}{s}}$, we not only make the expected number of samples polynomial in $s$, but also minimize the total number of calls to $\mathcal{V}$, as proven in Theorem \ref{thm:theorem_coarsen}. Please refer to the proof in Appendix \ref{appendix:proof_stats}.

% \begin{theorem}
% \label{thm:theorem_coarsen}
% With probability $\theta$=$e^{-\frac{1}{s}}$, \textsc{Sample\_Coarsen} learns a minimal NAP specification with $\mathcal{O}(slog|N|)$ calls to $\mathcal{V}$.
% \end{theorem}

% Thu


% If $\theta$ is set to a constant value, then the expected number of samples needed to obtain one that can be verified is $(\frac{1}{\theta})^{s}$. 




% The challenge once again is setting $\theta$ such that the trials required until \(\mathcal{V}(a) = 1\) is not exponential to $|M|$. Consider a \(\theta^{|M|}\) probability of sampling a random set of neurons that proves the query. The expected number of trials until we prove the query is thus $(\frac{1}{\theta})^s$. On the other hand, when the sample can be verified, we reduce the number of components by a factor of \(\theta\). The trade-off arises as setting \(\alpha\) too small results in too many trials per iteration, but setting \(\alpha\) too large results in too many iterations. The following theorem shows how they can be balanced. Please refer to the proof in the Appendix \ref{appendix:proof_coarsen}.



% \begin{algorithm2e}[H]
%     \caption{\textsc{Sample\_Coarsen}}
%     \label{alg:samplecoarsen}
%     \small
%     \DontPrintSemicolon
%     \SetKwProg{Fn}{Function}{}{end}
%     \SetKwFunction{Coarsen}{Coarsen}
%     \KwIn{The neural network $N$, the probability $\theta$, and the size $s$}
%     \KwOut{A minimal NAP specification $P$}
    
%     % \Fn{Gradient\_Heuristics($unvisited$, $\theta$)}{
%     %     $P \leftarrow \dot{\mathcal{A}}(N)$ \tcc*{Use the coarsest NAP as a blank template}
%     %     \For{$N_{i, l}$ \textbf{in} $unvisited$}{
%     %         $rand \leftarrow \text{random}(0,1)$ \;
%     %         \uIf{$rand \leq \theta$}{
%     %             $P_{i,l} \leftarrow \widetilde{\mathcal{A}}(N_{i, l})$ \tcc*{Refine unvisited neurons using $\widetilde{\mathcal{A}}$ with probability $\theta$}
%     %         }
%     %     }
%     %     \Return $P$\;
%     % }
%     \Fn{Sample\_Coarsen($mand\_neurons$, $\theta$, $s$)}{
%     $P \leftarrow \widetilde{\mathcal{A}}(N)$; $mand\_neurons \leftarrow N$\;
%     \uIf{$\mathcal{V}(P) == 0$}{
%         \Return $None$ \tcc*{Return None if the most refined NAP fails verification}
%     }
%     \Else{
%         \While{$|P| > s$}{
%             $P \leftarrow Sample\_NAPs(mand\_neurons , \theta)$\;
%             \uIf{$\mathcal{V}(P) == 1$ }{ 
%                 $found\_neurons \leftarrow \emptyset$ \;
%                 \For{$N_{i, l}$ \textbf{in} $N$}{
%                     \uIf{$P_{i, l} == \widetilde{\mathcal{A}}(N_{i, l})$} {
%                         $found\_neurons  \leftarrow found\_neurons  \cup \{N_{i, l}\}$ 
%                     }
%                 }$mand\_neurons \leftarrow found\_neurons$  \tcc*{Reduce search space}
%             }
%             \Else{
%                 $P \leftarrow Sample\_Naps(mand\_neurons , \theta)$ \tcc*{Sample a new NAP}
%             }
%         }
%         \Return $P$ \tcc*{Return the minimal NAP of size $s$}
%     }
%     }

    
    
% \end{algorithm2e}

% \begin{theorem}
% \label{thm:theorem_coarsen}
% With probability $\theta$=$e^{-\frac{1}{s}}$, \textsc{Sample\_Coarsen} learns a minimal NAP specification with $\mathcal{O}(slog|N|)$ calls to $\mathcal{V}$.
% \end{theorem}

% We will include the proof in the appendix. 





% \textbf{Theorem 3 (Properties of \textsc{ActiveCoarsen})}. Let \(s\) be the size of the largest minimal abstraction. If we set the refinement probability \(\alpha = e^{-1/s}\), the expected number of calls to the analysis \(\mathcal{V}\) made by \textsc{ActiveCoarsen}(\(\mathbb{J}\)) is \(O(s \log |\mathbb{J}|)\).

% \rebecca{\begin{table}[h]
% \centering
% \begin{tabular}{lcccc}
% \toprule
% \textbf{dataset, model size} & \textbf{|\mathbb{J}|} & \textbf{ScanCoarsen} & \textbf{StatRefine} & \textbf{ActiveCoarsen} \\ 
% \midrule
% Iris (10*2)                 & 20            &                      &                     &                        \\
% Iris (20*3)                 & 60            & 1 (1.6\%)            & 6 (10\%)            & 1 (1.6\%)              \\
% Mnist (256*2)               & 512           &                      &                     &                        \\
% Mnist (256*4)               & 1024          &                      &                     &                        \\
% Mnist (256*6)               & 1536          &                      &                     &                        \\
% \bottomrule
% \end{tabular}
% \caption{\rebecca{Average minimal abstraction size}}
% \label{your-label-here}
% \end{table}}

% \paragraph{Setting the sample probability $\theta$} Setting $s$ poses a challenge in practice, as we assume that $s$ is always provided in \textsc{Sample\_Refine} and \textsc{Sample\_Coarsen}. However, this can be addressed by dynamically updating $\theta$ based on the result of $\mathcal{V}(P)$ \cite{minimal_abs}. With $\theta$ from theorem \ref{thm:theorem_coarsen}, \textsc{Sample\_Coarsen} finds a NAP specification with probability $\left( e^{-1/s} \right)^s = e^{-1}$. Recall that theorem \ref{thm:theorem_refine} state that \textsc{Sample\_Refine} finds a NAP specification with probability $\left( \frac{|M|}{|M|+1} \right)^{|M|}$. The probability approaches \( e^{-1} \) asymptotically. Thus, we aim to set $\theta$ such that the $Pr(\mathcal{V}(P)=1) = e^{-1}$. Intuitively, if a sampled NAP $P$ is a specification, we decrease $\theta$ so less neurons will be refined or more neurons will be coarsened. Similarly, if $P$ is not a specification, $\theta$ needs to be increased. 


% Given that $\theta \in [0,1]$, we can parameterize it using the Sigmoid function $\sigma(\lambda) = \left( 1 + e^{-\lambda} \right)^{-1}$, where $\lambda \in (-\infty,\infty)$. Since $Pr(\mathcal{V}(P)=1)$ depends on $\theta$ as well, we express it as a function of $\lambda$, \( g(\lambda) = Pr( \mathcal{V}(P) = 1) \). Then, setting $Pr(\mathcal{V}(P)=1) = e^{-1}$ can be achieved through the following minimization problem:

% \begin{equation}
%     L(\lambda) = \frac{1}{2}(g(\lambda) - e^{-1/s})^2
% \end{equation}

% The loss function $L(\lambda)$ can be minimized by statistical learning using stochastic gradient descent. With a step size \(\eta\), update $\lambda$ using $\lambda \leftarrow \lambda - \eta \frac{dL}{d\lambda} $. Note that $\frac{dL}{d\lambda}$ can be expressed as:

% \begin{equation}
%     {\frac{dL}{d\lambda}} = (g(\lambda) - e^{-1/s}) \frac{dg(\lambda)}{d\lambda}
% \end{equation}


% Given \( g(\lambda) = Pr( \mathcal{V}(P) = 1) \), we can replace $g(\lambda)$ with $\mathcal{V}(P)$ for stochastic gradient update. Additionally, since $\frac{dg(\lambda)}{d\lambda} > 0$, we simply ignore it as its multiplication effect can be represented by $\eta$.  Therefore, the final update rule is given by:
% \begin{equation}
% \lambda \leftarrow \lambda - \eta(\mathcal{V}(P) - e^{-1})
% \end{equation}


% Where $\eta$ is the 
% Note that we have not verified the step size conditions that guarantee
% convergence. Instead, we simply set η = 0.1 for our experiments, which
% worked well in practice.

% In other words, if \( \mathcal{V}(P) = 1 \), we decrease \( \theta \). Otherwise we increase \( \theta \). 




% \subsection{Discussion of Algorithms}
% Table 1 provides an overview of the characteristics of the three algorithms discussed in our paper when applied to various datasets and model sizes. \\
% Properly configuring the parameter $\alpha$ for StatRefine and ActiveCoarsen is crucial as it introduces randomness, significantly impacting the formation of a well-structured NAP. \\
% Specifically, while StatRefine operates with a fixed runtime, there's no assurance of finding the minimal NAP since the algorithm may explore a wide range of minimal NAPs with d-dependent components. On the other hand, ActiveCoarsen has random runtime, but it doesn't always guarantee the existence of a minimal NAP as it focuses on identifying one minimal NAP. \\
% Despite the trade-offs associated with using StatRefine and ActiveCoarsen, these learning-based algorithms offer certain advantages over the deterministic ScanCoarsen algorithm. Their sparse nature results in a logarithmic dependency on $|\mathbb{J}|$, potentially leading to increased efficiency.











% \begin{definition}[Neural Activation Pattern] A \emph{Neural Activation Pattern (NAP)} of a neural network $\cN$ is a pair $\cP_\cN \mathbin{:=} (A, D)$, where $A$ and $D$ are two disjoint set of neurons.
% \end{definition}










% Essentially, $\delta$ controls the precision-recall trade-off for the NAP. Note that a slight decrease in $\delta$, such as 0.99, can already have a huge effect: a neuron may be activated in 99\% of the input, but the collection of all said neurons\xx{"said"?} is only activated together in 79\% of the input (775 out of 980), as can be seen with label 0 in \cref{tab:mnist_test_count}.

% \allen{more fix}







% Intuitively, for each neuron, we ask: how often is this neuron activated/deactivated upon seeing inputs from a label $l$. $\delta$ controls how precise we want to be: should we add a neuron to our NAP only if it is activated in all the inputs labeled $\ell$, or 95\% of the inputs is enough?
% \input{nap_input_alignment.tex}
% Thus, as $\delta$ \st{increases}\xx{decreases}, we expect the size of NAPs \st{also}\xx{remove also} to increase. Choosing the right $\delta$ has a huge impact on how useful the relaxed dominant NAPs can be. 
% \cref{tab:mnist_test_count} gives us some intuition why. For MNIST, the table shows how many test images from a label $\ell$ follow $\cP^\delta_\ell$, together with how many test images from other labels that also follow the same $\cP^\delta_\ell$.
% For example, there are 980 images in the test set with label 0 (second column). Among them, 967 images follow $\cP^{\delta=1.0}_{\ell=0}$. In addition to that, there are 20 images from the other 9 labels that also follow $\cP^{\delta=1.0}_{\ell=0}$. 
% % for the first big column for  0 consists two sub-columns $0$ and $\overline{0}$, 967 test images from class 0 and 20 test images from class $\overline{0}$, i.e. classes 1-9, misclassified as 0 follow the $\NAP$ at $\delta=0.0$. 
% With the \st{increase} \xx{decrease} of $\delta$, we can see that in both cases, both numbers decrease, suggesting that it is harder for an image to follow $\cP^{\delta=1.0}_{\ell=0}$ without being classified as 0 (the NAP is more precise), at the cost of having many images classified as 0 fail to follow $\cP^{\delta=1.0}_{\ell=0}$ (the NAP recalls worse). Essentially, $\delta$ controls the precision-recall trade-off for the NAP. Note that a slight decrease in $\delta$, such as 0.99, can already have a huge effect: a neuron may be activated in 99\% of the input, but the collection of all said neurons\xx{"said"?} is only activated together in 79\% of the input (775 out of 980), as can be seen with label 0 in \cref{tab:mnist_test_count}.
% \allen{rewrite and fix}

% the number of test images following the $\NAP$ decreases, especially for the class $\overline{i}$ case, the number drops dramatically when increasing $\delta$ from 0.00 to 0.01. 



% For the rest of the paper, if not explicitly stated, we refer to the $\delta$-relaxed dominant 
%  NAPs when talking about NAPs. When the context is clear, we drop any of the $\delta, \cN \text{and } \ell$ from the notation for clarity.

% \input{MarabouExample.tex}





% While in Simplex, a violation can only happen due to a variable becoming out-of-bound, in Marabou a violation can also happen when a variable doesn't satisfy its activation constraints.



% \subsection{Marabou}
% \ag{Remove unnecessary discussion of what could be used. Focus on Marabou only.}
% In theory, any SMT solver (e.g Z3 \citep{z3}, CVC5 \citep{cvc5}) can be used to solve the adversarial attacks and the robustness verification problem: the network and the properties can both be encoded as optimization problems over a set of linear constraints (the weighted sum and the properties) and non-linear constraints (the activation function). For example, \cref{fig:marabou_consts} shows how to encode the property that XNET is 0.04-robust at (0.06, 0.06), which then can be verified by both Z3 and CVC5. In practice, dedicated neural network verifiers are needed to verify any network of non-trivial size: by exploiting neural networks' properties with heuristics that may not be applicable in the general SMT setting, dedicated NN verifiers can be a few orders of magnitude faster than general-purpose solver \citep{abc}.



% By focusing only on neural networks with piecewise-linear activation functions, Marabou makes two insights: first, only a small subset of the activation nodes are relevant to the property under consideration. Hence, Marabou treats the non-linear constraints lazily and reduces the number of expensive case-splits, making it much faster than traditional SMT solvers. Second, Marabou repeatedly refines each variable's lower and upper bound, hoping that many piecewise-linear constraints can be turned into linear (phase-fixed), reducing further the need for case splitting. Altogether, Marabou achieves state-of-the-art performance on a wide range of benchmarks \cite{vnncomp2021}.

==> lonenorm.tex <==
\begin{figure}[!htb]
         \centering        \includegraphics[width=0.75\textwidth]{figures/mnist_L1_no_outliers.pdf}
         \caption{The distribution of $L_1$-norms of all image pairs for each class.}
         \label{fig:mnist_L1}
\end{figure}

==> marabou_mnist.tex <==


\begin{table}[t]
\caption{The maximum overlap ratio of dominant pattern for each label (class) on a given $\delta$ for MNIST. Each cell is obtained by $\max_i |N_{col}^{\delta} \bigcap N_i^{\delta}|/ |N_{col}^{\delta}|$ where $N_{col}^{\delta}$ is the set of neurons in the dominant pattern for the label (class) in the header of the column of the selected cell with the given $\delta$, $N_i$ is the set of neurons in the dominant pattern for the label (class) $i$ with the given $\delta$.} 
\label{tab:mnist_max_overlap_ratio}
\begin{center}
\begin{tabular}{ |c || c c c c c c c c c c| }
 \hline
& label0& label1& label2& label3& label4& label5& label6& label7& label8&label9\\
\hline\hline
0.000&0.959 &0.928 &0.963 &0.966 &0.972 &0.973 &0.930 &0.965 &0.957 &0.981\\ 
 \hline
0.010&0.844 &0.834 &0.911 &0.901 &0.881 &0.898 &0.895 &0.884 &0.880 &0.908\\ 
 \hline
0.050&0.864 &0.885 &0.909 &0.904 &0.915 &0.908 &0.899 &0.897 &0.890 &0.893\\ 
 \hline
0.100&0.877 &0.900 &0.910 &0.901 &0.921 &0.910 &0.890 &0.899 &0.900 &0.901\\ 
 \hline
0.150&0.876 &0.904 &0.904 &0.900 &0.919 &0.913 &0.893 &0.907 &0.904 &0.900\\ 
 \hline
0.250&0.893 &0.922 &0.913 &0.912 &0.928 &0.925 &0.905 &0.916 &0.916 &0.913\\ 
 \hline
0.500&0.903 &0.905 &0.925 &0.923 &0.926 &0.923 &0.907 &0.918 &0.927 &0.927\\ 
 \hline
\end{tabular}
\end{center}
\end{table}


==> misclsfy_fig_tex/FigMisclassify0.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred0_gt5_idx323.pdf}
         \caption{A testing image from MNIST with ground truth 5, classified as 0}
         \label{fig:misclsfy_5_to_0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred0_gt8_idx467.pdf}
         \caption{A testing image from MNIST with ground truth 8, classified as 0}
         \label{fig:misclsfy_8_to_0}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred0_gt9_idx665.pdf}
         \caption{A testing image from MNIST with ground truth 9, classified as 0}
         \label{fig:misclsfy_9_to_0}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 0 and also follow the $\NAP$ of class 0.}
        \label{fig:Misclassify_to_0}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify1.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt6_idx438.pdf}
         \caption{A testing image from MNIST with ground truth 6, classified as 1}
         \label{fig:misclsfy_6_to_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt7_idx129.pdf}
         \caption{A testing image from MNIST with ground truth 7, classified as 1}
         \label{fig:misclsfy_7_to_1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred1_gt9_idx229.pdf}
         \caption{A testing image from MNIST with ground truth 9, classified as 1}
         \label{fig:misclsfy_9_to_1}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 1 and also follow the $\NAP$ of class 1.}
        \label{fig:Misclassify_to_1}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify2.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred2_gt1_idx348.pdf}
         \caption{A testing image from MNIST with ground truth 1, classified as 2}
         \label{fig:misclsfy_1_to_2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred2_gt3_idx305.pdf}
         \caption{A testing image from MNIST with ground truth 3, classified as 2}
         \label{fig:misclsfy_3_to_2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred2_gt7_idx915.pdf}
         \caption{A testing image from MNIST with ground truth 7, classified as 2}
         \label{fig:misclsfy_7_to_2}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 2 and also follow the $\NAP$ of class 2.}
        \label{fig:Misclassify_to_2}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify3.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred3_gt5_idx184.pdf}
         \caption{A testing image from MNIST with ground truth 5, classified as 3}
         \label{fig:misclsfy_5_to_3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred3_gt7_idx396.pdf}
         \caption{A testing image from MNIST with ground truth 7, classified as 3}
         \label{fig:misclsfy_7_to_3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred3_gt9_idx343.pdf}
         \caption{A testing image from MNIST with ground truth 9, classified as 3}
         \label{fig:misclsfy_9_to_3}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 3 and also follow the $\NAP$ of class 3.}
        \label{fig:Misclassify_to_3}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify4.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred4_gt2_idx398.pdf}
         \caption{A testing image from MNIST with ground truth 2, classified as 4}
         \label{fig:misclsfy_2_to_4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred4_gt6_idx488.pdf}
         \caption{A testing image from MNIST with ground truth 6, classified as 4}
         \label{fig:misclsfy_6_to_4}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred4_gt9_idx364.pdf}
         \caption{A testing image from MNIST with ground truth 9, classified as 4}
         \label{fig:misclsfy_7_to_2}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 4 and also follow the $\NAP$ of class 4.}
        \label{fig:Misclassify_to_4}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify5.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred5_gt3_idx39.pdf}
         \caption{A testing image from MNIST with ground truth 3, classified as 5}
         \label{fig:misclsfy_3_to_5}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred5_gt6_idx102.pdf}
         \caption{A testing image from MNIST with ground truth 6, classified as 5}
         \label{fig:misclsfy_6_to_5}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred5_gt8_idx288.pdf}
         \caption{A testing image from MNIST with ground truth 8, classified as 5}
         \label{fig:misclsfy_8_to_5}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 5 and also follow the $\NAP$ of class 5.}
        \label{fig:Misclassify_to_5}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify6.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred6_gt0_idx139.pdf}
         \caption{A testing image from MNIST with ground truth 0, classified as 6}
         \label{fig:misclsfy_0_to_6}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred6_gt2_idx357.pdf}
         \caption{A testing image from MNIST with ground truth 3, classified as 6}
         \label{fig:misclsfy_2_to_6}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred6_gt5_idx871.pdf}
         \caption{A testing image from MNIST with ground truth 5, classified as 6}
         \label{fig:misclsfy_5_to_6}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 6 and also follow the $\NAP$ of class 6.}
        \label{fig:Misclassify_to_6}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify7.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred7_gt2_idx35.pdf}
         \caption{A testing image from MNIST with ground truth 2, classified as 7}
         \label{fig:misclsfy_2_to_7}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred7_gt3_idx173.pdf}
         \caption{A testing image from MNIST with ground truth 3, classified as 7}
         \label{fig:misclsfy_3_to_7}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred7_gt9_idx980.pdf}
         \caption{A testing image from MNIST with ground truth 9, classified as 7}
         \label{fig:misclsfy_9_to_7}
     \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 7 and also follow the $\NAP$ of class 7.}
        \label{fig:Misclassify_to_7}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify8.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred8_gt1_idx74.pdf}
         \caption{A testing image from MNIST with ground truth 1, classified as 8}
         \label{fig:misclsfy_1_to_8}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred8_gt3_idx593.pdf}
         \caption{A testing image from MNIST with ground truth 3, classified as 8}
         \label{fig:misclsfy_3_to_8}
     \end{subfigure}
     % \hfill
     % \begin{subfigure}[t]{0.3\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred7_gt9_idx980.pdf}
     %     \caption{A testing image from MNIST with ground truth 9, classified as 7}
     %     \label{fig:misclsfy_9_to_7}
     % \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 8 and also follow the $\NAP$ of class 8.}
        \label{fig:Misclassify_to_8}
\end{figure}

==> misclsfy_fig_tex/FigMisclassify9.tex <==
\begin{figure}[th]
     \centering
     \begin{subfigure}[t]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred9_gt4_idx231.pdf}
         \caption{A testing image from MNIST with ground truth 4, classified as 9}
         \label{fig:misclsfy_4_to_9}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.4\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred9_gt7_idx134.pdf}
         \caption{A testing image from MNIST with ground truth 7, classified as 9}
         \label{fig:misclsfy_7_to_9}
     \end{subfigure}
     % \hfill
     % \begin{subfigure}[t]{0.3\textwidth}
     %     \centering
     %     \includegraphics[width=\textwidth]{figures/mnist_interesting_samples/eps0-0_pred7_gt9_idx980.pdf}
     %     \caption{A testing image from MNIST with ground truth 9, classified as 7}
     %     \label{fig:misclsfy_9_to_7}
     % \end{subfigure}
        \caption{Some interesting test images from MNIST that are misclassified as 9 and also follow the $\NAP$ of class 9.}
        \label{fig:Misclassify_to_9}
\end{figure}

==> nap_augmented_prop.tex <==
\begin{table}[t]
\caption{MOVE TO APPENDIX! Searching for adversarial examples for each label within the $L_\infty$ norm-balls of radius 0.1 ($\epsilon = 0.1$) centered at 0. Each column represents a label to be checked. The first row doesn't take NAPs into consideration, the remaining rows use NAPs of different $\delta$s. We report Y if no adversarial examples are found, N otherwise. }

\allen[Be careful with the meaning of Y and N.]
\label{tab:effect_of_delta}
\begin{center}
\begin{tabular}{ |l || r r r r r r r r r r| }
 \hline
& 0& 1& 2& 3& 4& 5& 6& 7& 8& 9\\
\hline\hline
$\epsilon = 0.1$&N &N &N &N &N &N &N &N &N &N \\  
 \hline
$\epsilon = 0.1, \delta = 0.00$&N &N &N &N &N &N &N &N &N &N \\  
 \hline
$\epsilon = 0.1, \delta = 0.01$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.05$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.10$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.15$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta = 0.25$&N &N &N &N &N &N &N &N &N &N \\ 
\hline
$\epsilon = 0.1, \delta =0.50$&\Y &\Y &\Y &N &\Y &\Y &\Y &\Y &\Y &\Y \\ 
\hline

\end{tabular}
\end{center}
\end{table}


==> nap_input_alignment.tex <==
\begin{table*}[t]
\caption{The number of the test images in MNIST that follow a given $\NAP^\delta$. For a label $i$, $\overline{i}$ represents images with labels other than $i$ yet follow $\NAP^\delta_{\ell=i}$. The leftmost column is the values of $\delta$. The top row indicates how many images in the test set are of a label. } 
\label{tab:mnist_test_count}
\vskip 0.1in
\begin{center}
% \tiny
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ |l ||r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r| }
\hline
& \multicolumn{2}{r|}{0}& \multicolumn{2}{r|}{1}& \multicolumn{2}{r|}{2}& \multicolumn{2}{r|}{3}& \multicolumn{2}{r|}{4}& \multicolumn{2}{r|}{5}& \multicolumn{2}{r|}{6}& \multicolumn{2}{r|}{7}& \multicolumn{2}{r|}{8}& \multicolumn{2}{r|}{9}\\
& \multicolumn{2}{r|}{(980)}& \multicolumn{2}{r|}{(1135)}& \multicolumn{2}{r|}{(1032)}& \multicolumn{2}{r|}{(1010)}& \multicolumn{2}{r|}{(982)}& \multicolumn{2}{r|}{(892)}& \multicolumn{2}{r|}{(958)}& \multicolumn{2}{r|}{(1028)}& \multicolumn{2}{r|}{(974)}& \multicolumn{2}{r|}{(1009)}\\
\cline{2-21}
&&&&&&&&&&&&&&&&&&&&\\[-0.9em]
&0 & $\overline{0}$ & 1 & $\overline{1}$ & 2 & $\overline{2}$ & 3 & $\overline{3}$ & 4 & $\overline{4}$ & 5 & $\overline{5}$ & 6 & $\overline{6}$ & 7 & $\overline{7}$ & 8 & $\overline{8}$ & 9 & $\overline{9}$\\
\hline\hline
1.00&967 & 20 & 1124 & 8 & 997 & 22 & 980 & 13 & 959 & 25 & 874 & 32 & 937 & 26 & 1003 & 28 & 941 & 22 & 967 & 12\\ 
 \hline
0.99&775 & 1 & 959 & 0 & 792 & 4 & 787 & 2 & 766 & 3 & 677 & 1 & 726 & 4 & 809 & 2 & 696 & 3 & 828 & 4\\ 
 \hline
0.95&376 & 0 & 456 & 0 & 261 & 1 & 320 & 0 & 259 & 0 & 226 & 0 & 200 & 0 & 357 & 0 & 192 & 0 & 277 & 0\\ 
 \hline
0.90&111 & 0 & 126 & 0 & 43 & 0 & 92 & 0 & 76 & 0 & 24 & 0 & 45 & 0 & 144 & 0 & 44 & 0 & 73 & 0\\ 
 \hline
\end{tabular}%
}
\end{center}
\end{table*}


==> nap_volume.tex <==
\section{Volume Estimation of $R_{P}$}
\label{appendix: nap volume}



% \section{Calculating(approximating) verifiable volumn}
% \textbf{Working with NAPs using Marabou} In this paper, we use Marabou \citep{Marabou}, a dedicated state-of-the-art NN verifier. Marabou extends the Simplex \cite{simplex} algorithm for solving linear programming with special mechanisms to handle non-linear activation functions. Internally, Marabou encodes both the verification problem and the adversarial attacks as a system of linear constraints (the weighted sum and the properties) and non-linear constraints (the activation functions). Same as Simplex, at each iteration, Marabou tries to fix a variable so that it doesn't violate its constraints. While in Simplex, a violation can only happen due to a variable becoming out-of-bound, in Marabou a violation can also happen when a variable doesn't satisfy its activation constraints.

% NAPs and NAP properties can be encoded using Marabou with little to no changes to Marabou itself. To force a neuron to be activated or deactivated, we add a constraint for its output. To improve performance, we infer ReLU's phases implied by the NAPs, and change the corresponding constraints\footnote{Marabou has a similar optimization, but the user cannot control when or if it is applied.}.For example, given a ReLU $v_i=max(v_k, 0)$, to enforce $v_k$ to be activated, we remove the constraint from Marabou and add two new ones: $v_i = v_k$, and $v_k \geq 0$.


\begin{wrapfigure}{R}{0.4\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/volume.pdf}
  \caption{Volume Estimation of \( R_{P} \) using an orthotope in a 2-dimensional case. The gray rectangle represents the input space, with the training set depicted by a collection of data points \( + \). The polygon corresponds to some NAP \( P \). Initially, we identify an anchor point, denoted by \textcolor{red}{\( + \)}. Then, we construct the orthotope, represented by the green rectangle, by extending upper and lower bounds starting from the anchor point until it extends beyond \( P \).}
  \label{fig:volume}
\end{wrapfigure}


Conceptually, NAP specifications typically correspond to significantly larger input regions compared to local neighbourhood specifications. This serves as the primary motivation for utilizing NAPs as specifications. However, previous work lacks sufficient justification or evidence to support this claim. In this section, we propose a simple method for approximating the volume of $R_{P}$, i.e., the region corresponding to a NAP $P$. This allows us to: 1) quantify the size difference between $R_{P}$ and $L_\infty$ ball specifications; 2) gain insights into the volumetric change from the most refined NAP specification to the minimal NAP specification.

Computing the exact volume of $R_{P}$ is at least NP-hard, as determining the exact volume of a polygon is known to be NP-hard \cite{volume_np}. Moreover, computing the exact volume of $R_{P}$ can be even more challenging due to its potential concavity. To this end, our method estimates the volume of $R_{P}$ by efficient computation of an orthotope that closely aligns with $R_{P}$, as illustrated in Figure \ref{fig:volume}. We briefly describe it as follows:


% Computing the exact volume of $R_{P}$ is at least NP-hard, as determining the exact volume of a polygon is known to be NP-hard \cite{volume_np}. Moreover, computing the exact volume of $R_{P}$ can be even more challenging due to its potential concavity. In our approach, we tackle this challenge by estimating the volume of $R_{P}$ through the efficient computation of an orthotope that closely approximates $R_{P}$, as depicted in Figure \ref{fig:volume}. We outline our method briefly as follows:









% \subsection{Volume Comparison Between $R_{P}$ and $L_\infty$ Balls }
% \subsection{Volume Comparison Between the Most Refined and the Minimal NAP Specification  }

% \begin{figure}[H]
%   \centering
%   \includegraphics[width=0.5\textwidth]{figures/volume.pdf}
%   \caption{Volume Estimation of \( R_{P} \) using an orthotope in a 2-dimensional case. The gray rectangle represents the input space, with the training set depicted by a collection of data points \( + \). The polygon corresponds to some NAP \( P \). Initially, we identify an anchor point, denoted by \textcolor{red}{\( + \)}. Then, we construct the orthotope, represented by the green rectangle, by extending upper and lower bounds starting from the anchor point until it extends beyond \( P \).
% }
%   \label{fig:volume}
% \end{figure}

% \begin{algorithm2e}[H]
%     \caption{\textsc{Estimate\_Volume}}
%     \label{alg:volume_comparison}
%     \small
%     \DontPrintSemicolon
    
    % \SetKwProg{Fn}{Function}{}{end}
    % \SetKwFunction{Binary_Search}{Find_Center}
    % \KwOut{The point, $C$, that is the  $L_{\infty}$ radius}
    % \Fn{Find\_Center($X$)}{
    %     $Center$ $\leftarrow$ $X[0]$\;
    %   \While{$Center$ does not center at the $L_{\infty}$ Ball contains $X.random\_sample()$}
    %   {
    %     $Center \leftarrow$ center of $X.random\_sample().L_{\infty}$center\;
    %   }
    % \Return $Center$
    % }
    % \SetKwProg{Fn}{Function}{}{end}
    % \SetKwFunction{Binary_Search}{Binary_Search}
    % \Fn{Binary\_Search($lw$, $ub$, $P$)}{
    %   \While{$ub-lb > \epsilon$}{
    %     $mid$ $\leftarrow$ $(ub+lb)/2$\;
    %   \lIf{$P$ still holds after extending $lb$ to $mid$}{$lb \leftarrow mid$}
    %   \lElse{$ub \leftarrow mid$}
    %   }

    % \Return $mid$
    % }    
%     \SetKwProg{Fn}{Function}{}{end}
%     \SetKwFunction{Estimate Volume}{Estimate Volume}
%     \KwIn{A NAP $P$, a set of data $D$, which can be verified by $P$, and the model $M$}
%     \KwOut{The estimated volume of the input space around the center $C$, which can be verified by $P$}
%     \Fn{Estimate\_Volume($P$, $X$, $D$)}{
%     $Volume$ $\leftarrow$ $\emptyset$\;
%     $C \leftarrow Find\_Center(X)$\;
%   \For{$c \in C$}{
%     $ub \gets$ Binary\_Search($c$, 1, $P$) \tcp*{Extend to upper bound}
%     $lb \gets$ Binary\_Search(0, $c$, $P$) \tcp*{Extend to lower bound}
%     $Volume$.Append($ub-lb$)
%   }
%     \Return $Volume$
%     }   
% \end{algorithm2e}

% The procedures for estimating the ratio between the volumes of the input spaces correspond to the minimal and most refined NAP's are:
% \noindent \begin{wrapfigure}{r}{0.35\textwidth}
%   \centering
%   \vspace{50pt}
%   \includegraphics[width=0.35\textwidth]{figures/volume.pdf}
%   \caption{The Triangle represents the input data space, , denoted by $P_m$, corresponds to the minimal NAP. and the inside polygon corresponds to the most refined NAP, denoted by $P_r$. d$_0$ and d$_1$ are the input data dimensions. The green and gray rectangles are the estimated areas.}
%   \label{fig:volumn}
% \end{wrapfigure}


\paragraph{Finding an anchor point} The first step is to find an anchor point to serve as the center of the orthotope. Ideally, this anchor point should be positioned close to the center of $R_{P}$ to ensure a significant overlap between the orthotope and $R_{P}$. However, computing the actual center of $R_{P}$ is costly. Thus, we look for a pseudo-center from the training set $X$ that resides in $R_{P}$. This pseudo-center can be computed by finding the point that uses the smallest $L_{\infty}$ ball to cover other data points, solved as the following optimization problem:
\[
c_{\text{pseudo}} = \underset{x \in R_{P}}{\arg\min} \max_{x' \in  R_{P}} \|x - x'\|_{\infty}
\]
where $R_{P} = \{ x \mid \mathcal{A}(N,x) \preccurlyeq P, x \in X \}$. When $|X|$ is small, $c_{\text{pseudo}}$ can be computed directly; for larger $|X|$, a statistical computation strategy is required.

\paragraph{Constructing the orthotope} Once the pseudo-center \( c_{\text{pseudo}} \) is determined, we want to create an orthotope around \( c_{\text{pseudo}} \) to closely align with \( R_{P} \). The orthotope is constructed by determining pairs of upper and lower bounds \( U^{(i)} \) and \( L^{(i)} \) for each dimension \( i \). Specifically, \( U^{(i)} \) and \( L^{(i)} \) are computed through expansion in two opposite directions from \( c_{\text{pseudo}} \) along dimension \( i \) until they extend beyond \( R_{P} \). This expansion can be expressed as:

\[
\max_{U^{(i)}} \{ x' \in R_{P} \,|\, x' := c_{\text{pseudo}} + U^{(i)} \}
\text{ ; }
\max_{L^{(i)}} \{ x' \in R_{P} \,|\, x' := c_{\text{pseudo}} - L^{(i)} \}
\]

Here, \( U^{(i)} \) and \( L^{(i)} \) represent the upper and lower bounds in dimension \( i \) respectively, originating from \( c_{\text{pseudo}} \). These bounds can be efficiently calculated with binary search.

The choice of the archer point is crucial in our approach. If it is located at a corner of \( R_p \), the volume calculation will be highly biased. This can pose a problem when we seek to understand the volumetric change from the most refined NAP specification to the minimal NAP specification. Additionally, using the orthotope as an estimator provides convenience in understanding the volumetric change simply by examining differences in each input dimension.

% \[
% \max_{ub} \{c_{\text{pseudo}} + ub | c_{\text{pseudo}} + ul \in R_{P}\}
% \]
% \[
% \max_{ul} \{c_{\text{pseudo}} + ul | c_{\text{pseudo}} + ul \in R_{P}\}
% \]


% in each dimension as much as possible until it reaches outside of $R_{P}$. 
%  \begin{equation*}
% \max_{\mathbf{d}} \quad \text{subject to} \quad \left( \forall \mathbf{x'} \in R_{P} : \| \mathbf{c_{\text{pseudo}}} - \mathbf{x'} + \mathbf{d} \|_{\infty} \leq \epsilon \right)
% \end{equation*}

% As the distance metric becomes invalid in hih-dimensional space,


% We chose it from the given training data set $X$, 

% Recall the region is defined as $R_{P}= \{ x \mid {\mathcal{A}(N,x) \preccurlyeq P}  \}  $. 




% \begin{enumerate}
%     \item Intuitively, the estimated center should live in the space corresponds to a most refined NAP and close to the real center of the space for the corresponding minimal NAP. Therefore, as demonstrated in Figure\ref{fig:volumn}, the estimated center is chosen from a sample of $P_r$ and should cover a sample of $P_m$ with the least L$_{\infty}$ ball.
%     \item  For each dimension of the estimated center, we verify how much can this dimension increase or decrease so that it can still satisfy the NAP. These bounds could be found efficiently through binary search. As demonstrated in Figure\ref{fig:volumn}, the green shaded area is the least rectangle defined by such bounds, and can be seen as an estimated area for the most refined NAP. Likewise, the gray area is for the minimal NAP.
%     \item From the most refined to minimal NAP, the bounds/range of each dimension found in the last step may increase with some ratio. The product of these ratios is, as shown in Figure\ref{fig:volumn}, a good estimation of the volume ratio between the actual spaces.
% \end{enumerate}

% Given a most refined or minimal NAP, it is difficult to compute the accurate volume corresponds to this NAP. Therefore, we propose a metric aimed at estimating and comparing their volumes. The metric requires some way of expanding the area around a point until it no longer satisfies the NAP. Thus, an estimated center, as highlighted red in Figure\ref{fig:volumn}, is good for volume estimation because it has more space around it for the expansion.\\
% In order to find such estimated center, we first sample $n$ points from the input space corresponds to a minimal NAP. The goal is to find a point such that it can cover the other points through a $L_{\infty}$ Ball with the least radius. This process takes $\mathcal{O}$($n^2$) since it compares every pair of points.\\
% For each dimension of $C$, we compute for its maximal range that still satisfies the NAP with the other dimensions fixed. This allows us to know how spacious this point's surrounding is in these directions. In a 2-dimensional example as shown in Figure\ref{fig:volumn}, the red center moves horizontally in the $x_1$ direction or vertically until it reaches to the edge of the NAP specification. The green shaded area is the least rectangle containing the horizontal and vertical line extension corresponds to the most refined NAP. Similarly, the gray area is the space estimation of the minimal NAP. Although the estimation is not a bound of the actual area, the ratio between the ranges of the most refined and minimal NAP's allows us to know how much the space grows after minimizing a refined NAP with Marabou. Multiplying all these ratios, we get an estimated ratio of how much the space grows overall.

==> table_case_study.tex <==
% \begin{table}[t]
% \caption{The frequency of each ReLU and the dominant NAPs for each label. Activated and deactivated neurons are denoted by $+$ and $-$, respectively, and $*$ denotes an arbitrary neuron state.} 
% \label{tab:case_study}
% \centering
% \begin{tabular}{ l | r | c| r}
% \bf Label & \bf Neuron states & \bf \#samples & \bf Dominant NAP \\
% \hline
% \hline
% \multirow{2}{*}{0 (Green)}&$(+,-,-,+,-,+)$&8& \multirow{2}{*}{$(+,*,-,+,-,+)$} \\ 
%  %\cline{2-3}
% &$(+,+,-,+,-,+)$&2&  \\ 
%  \hline
% \multirow{3}{*}{1 (Red)}&$(+,+,-,-,+,-)$&7&  \multirow{3}{*}{$(*,+,-,+,-,*)$}\\ 
% %\cline{2-3}
% &$(-,+,-,-,+,-)$&2& \\ 
% % \cline{2-3}
% &$(+,+,-,-,+,+)$&1& \\ 
%  \hline

% \end{tabular}
% \end{table}

\begin{table}[th]
\caption{The frequency of each ReLU and the NAPs for each label. Activated and deactivated neurons are denoted by $+$ and $-$, respectively, and $*$ denotes an arbitrary neuron state.} 
\label{tab:case_study}
\vskip 0.1in
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ l | c | c| c}
\bf Label & \bf Neuron states & \bf \#samples & \bf NAP \\
\hline
\hline
\multirow{2}{*}{0 (Green)}&$(+,-,-,+,-,+)$&8& \multirow{2}{*}{$(+,*,-,+,-,+)$} \\ 
 %\cline{2-3}
&$(+,+,-,+,-,+)$&2&  \\ 
 \hline
\multirow{3}{*}{1 (Red)}&$(+,+,-,-,+,-)$&7&  \multirow{3}{*}{$(*,+,-,+,-,*)$}\\ 
%\cline{2-3}
&$(-,+,-,-,+,-)$&2& \\ 
% \cline{2-3}
&$(+,+,-,-,+,+)$&1& \\ 
 \hline

\end{tabular}
}
\end{table}


==> table_cifar10.tex <==
% at delta =0.05
% 1783	0.012	 unsat
% 6413	0.012	 sat
% 1189	0.012	 unsat
% 8498	0.012	 sat
% 7076	0.012	 unsat
% 1783	0.024	 TIMEOUT
% 6413	0.024	 sat
% 1189	0.024	 unsat
% 8498	0.024	 sat
% 7076	0.024	 sat
% 596	0.024	 TIMEOUT
% 9228	0.024	 unsat

% at delta =0.1
% 1783	0.012	 unsat
% 6413	0.012	 unsat
% 1189	0.012	 unsat
% 8498	0.012	 sat
% 7076	0.012	 unsat
% 1783	0.024	 unsat
% 6413	0.024	 unsat
% 1189	0.024	 unsat
% 8498	0.024	 sat
% 7076	0.024	 sat
% 596	0.024	 unsat
% 9228	0.024	 unsat


